Damping to prevent the blow-up of the Korteweg-de Vries equation

We study the behavior of the solution of a generalized damped KdV equation $u_t + u_x + u_{xxx} + u^p u_x + \mathscr{L}_{\gamma}(u)= 0$. We first state results on the local well-posedness. Then when $p \geq 4$, conditions on $\mathscr{L}_{\gamma}$ are given to prevent the blow-up of the solution. Finally, we numerically build such sequences of damping.

==> schemas.tex <==
The schemes were introduced in the paper [CheSad]. We remind that the schemes are implicits, so we need to use a Picard iterate to solve them. However, this brings some stability issues even if the schemes are unconditionally stable. We study here the stability of the schemes with the classic Picard iterate method. To simplify the writings, we denote $\widehat{u_n}(\xi)$ by $\widehat{u_n}$.

\subsection{Crank-Nicolson scheme}
	Let us remind the Crank-Nicolson scheme
	
	\[ \widehat{u_{n+1}} = \frac{1 - \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \widehat{u_n} - \frac{i\xi \frac{\Delta t}{2}}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \left( \frac{\widehat{u_{n+1}^{p+1}}}{p+1} + \frac{\widehat{u_{n}^{p+1}}}{p+1} \right).\]
	
	In the Picard iterate, we have 
	
	\[ \widehat{u_{n+1,r+1}} = \frac{1 - \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \widehat{u_n} - \frac{i\xi \frac{\Delta t}{2}}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \left( \frac{\widehat{u_{n+1,r}^{p+1}}}{p+1} + \frac{\widehat{u_{n}^{p+1}}}{p+1} \right).\]
	
	If a stopping condition is checked (generally $\| \widehat{u_{n+1,r+1}} - \widehat{u_{n+1,r+1}} \| < \epsilon$), $\widehat{u_{n+1,r+1}} =: \widehat{u_{n+1}}$.
	
	Consequently, 
	
	\[ \widehat{u_{n+1,r+1}} - \widehat{u_{n+1}} = \frac{i\xi \frac{\Delta t}{2}}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \left( \frac{\widehat{u_{n+1}^{p+1}}}{p+1} - \frac{\widehat{u_{n+1,r}^{p+1}}}{p+1} \right). \]
	
	This expression is not linear, so we can study the stability as we are used to. To be able to do it anyway, we linearise around $u_n$. First, 
	\[ \widehat{u_{n+1,r}^{p+1}} - \widehat{u_{n+1}^{p+1}} = \sum\limits_{j=0}^{p} \mathscr{F} \left[ \left( u_{n+1,r} - u_{n+1} \right) u_{n+1,r}^j u_{n+1}^{p-j} \right]. \]
	By linearising around $u_n$, we have $u_{n+1,r}^j u_{n+1}^{p-j} \sim u_n^p$. Thus
	\[ \widehat{u_{n+1,r}^{p+1}} - \widehat{u_{n+1}^{p+1}} \approx \sum\limits_{j=0}^{p} \mathscr{F} \left[ \left( u_{n+1,r} - u_{n+1} \right) u_{n}^p \right]. \]
	It follows that
	\[ \widehat{u_{n+1,r+1}} - \widehat{u_{n+1}} \approx -\frac{i\xi \frac{\Delta t}{2}}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \mathscr{F} \left[ (u_{n+1,r} - u_{n+1}) u_n^p \right]. \]
	The inequality
	\[ \left| \frac{i\xi \frac{\Delta t}{2}}{1+\frac{\Delta t}{2}\gamma(\xi) + i \frac{\Delta t}{2} \left( \xi - \xi^3 \right)} \right| = \frac{\left| \xi \frac{\Delta t}{2} \right|}{\sqrt{\left( 1+\frac{\Delta t}{2}\gamma(\xi) \right)^2 + \left( \frac{\Delta t}{2} \left( \xi - \xi^3 \right) \right)^2}} \leq \left| \xi \frac{\Delta t}{2} \right| \]
	is true because $\gamma(\xi) \geq 0$. Consequently
	\[ \Normp{u_{n+1,r+1} - u_{n+1}}{2}^2 \lessapprox \int_{\R} \abs{\xi\frac{\Delta t}{2}} \abs{\mathscr{F}\left[ (u_{n+1,r} - u_{n+1})u_n^p \right] }^2d\xi.  \]
	
	Numerically, we have
	\[ \xi = \frac{2k\pi}{L}, \quad -\frac{N_x}{2} \leq \frac{N_x}{2}-1, \quad N_x = \frac{L}{\Delta x}. \]
	Hence
	\[ \abs{\xi \frac{\Delta t}{2}}^2 \leq \left( \frac{\Delta t}{2} \frac{\pi}{2L} \frac{2L}{\Delta x} \right)^2 =\left( \frac{\pi \Delta t}{\Delta x} \right)^2. \]
	Thus 
	\[ \Normp{u_{n+1,r+1} - u_{n+1}}{2} \lessapprox \frac{\pi \Delta t}{\Delta x} \Normp{u_n}{\infty}^p \Normp{u_{n+1,r}-u_{n+1}}{2}. \]
	To ensure the stability, the following inequality has to be true
	\[ \frac{\pi \Delta t}{\Delta x} \Normp{u_n}{\infty}^p < 1 \quad \mbox{~i.e.~} \quad \Delta t < \frac{\Delta x}{\pi \Normp{u_n}{\infty}^p}. \]
	
	
	
\subsection{The Sanz-Serna scheme}
	Let us remind the Sanz-Serna scheme
	
	\begin{multline*}
		\widehat{u_{n+1}} = \frac{1 - \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \widehat{u_n} \\
		- \frac{i\xi \frac{\Delta t}{2}}{2^{p+1} (p+1) \left(1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right) \right)} \mathscr{F} \left( (u_{n+1} + u_n)^{p+1} \right).
	 \end{multline*}
	 
	 In the Picard iterate 
	\begin{multline*}
		\widehat{u_{n+1,r+1}} = \frac{1 - \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)}{1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right)} \widehat{u_n} \\
		- \frac{i\xi \frac{\Delta t}{2}}{2^{p+1} (p+1) \left(1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right) \right)} \mathscr{F} \left( (u_{n+1,r} + u_n)^{p+1} \right).
	 \end{multline*}	 
	 Thus
	 \begin{multline*}
	 	\widehat{u_{n+1,r+1}} - \widehat{u_n} = \frac{i\xi\Delta t}{2^{p+1} (p+1) \left(1 + \frac{\Delta t}{2} \left( i\xi - i\xi^3 + \gamma(\xi) \right) \right)} \\
	 	\times \left[ \mathscr{F} \left[ (u_{n+1}+u_n)^{p+1} - (u_{n+1,r}+u_n)^{p+1} \right) \right]. 
	 \end{multline*}
	 
	 \underline{First}
	 \begin{align*}
	 	(u_{n+1}+u_n)^{p+1} & = \sum\limits_{j=0}^{p+1} \binom{p+1}{j} u_{n+1}^j u_n^{p+1-j}, \\
	 	(u_{n+1,r}+u_n)^{p+1} & = \sum\limits_{j=0}^{p+1} \binom{p+1}{j} u_{n+1,r}^j u_n^{p+1-j},
	 \end{align*}
	 Hence
	 \[ (u_{n+1}+u_n)^{p+1} - (u_{n+1,r}+u_n)^{p+1} = \sum\limits_{j=0}^{p+1} \binom{p+1}{j} \left( u_{n+1}^j - u_{n+1,r}^j \right) u_n^{p+1-j}. \]
	 
	 \underline{Second}
	 \[ u_{n+1}^j - u_{n+1,r}^j = (u_{n+1} - u_{n+1,r}) \sum\limits_{l=0}^{j-1} u_{n+1}^l u_{n+1,r}^{j-1-l}. \]
	 
	 \underline{Third} : Linearisation around $u_n$
	 \begin{align*}
	 	u_{n+1}^j - u_{n+1,r}^j & \approx (u_{n+1} - u_{n+1,r})u_n^{j-1}, \\
	 	(u_{n+1}+u_n)^{p+1} - (u_{n+1,r}+u_n)^{p+1} & \approx \sum\limits_{j=0}^{p+1} \binom{p+1}{j} (u_{n+1} - u_{n+1,r}) u_n^p, \\ 
	 		& \approx (u_{n+1} - u_{n+1,r}) u_n^p \sum\limits_{j=0}^{p+1} \binom{p+1}{j}, \\
	 		& \approx 2^{p+1} (u_{n+1} - u_{n+1,r}) u_n^p.
	 \end{align*}
	 
	 We can now compute the $L^2$-norm
	 \[ \Normp{\widehat{u_{n+1,r+1}}-\widehat{u_{n+1}}}{2}^2 \lessapprox \int_{\R} \abs{\frac{\xi \Delta t}{p+1}}^2 \abs{\mathscr{F} \left[ (u_{n+1}-u_{n+1,r})u_n^p \right]}^2 d\xi. \]
	 With the same arguments than for the Crank-Nicolson scheme, we obtain
	 \[ \Normp{u_{n+1,r+1}-u_{n+1}}{2} \lessapprox \frac{2\pi \Delta t}{(p+1)\Delta x} \Normp{u_n}{\infty}^p \Normp{u_{n+1,r}-u_{n+1}}{2}.  \]
	To ensure the stability, the following inequality has to be true
	\[ \frac{2\pi \Delta t}{(p+1)\Delta x} \Normp{u_n}{\infty}^p < 1 \quad \mbox{~i.e.~} \quad \Delta t < \frac{(p+1) \Delta x}{2\pi \Normp{u_n}{\infty}^p}. \]
	
	
	
	
\subsection{The forward Euler scheme}

	The scheme is
	\[ \widehat{u_{n+1}} = \frac{1}{1+\Delta t \left( i\xi -i\xi^3 +\gamma(\xi) \right)} \widehat{u_n} - \frac{\frac{i\xi \Delta t}{p+1}}{1+\Delta t \left( i\xi -i\xi^3 +\gamma(\xi) \right)} \widehat{u_{n+1}^{p+1}}. \]
	In the Picard iterate we have
	\[ \widehat{u_{n+1,r+1}} = \frac{1}{1+\Delta t \left( i\xi -i\xi^3 +\gamma(\xi) \right)} \widehat{u_n} - \frac{\frac{i\xi \Delta t}{p+1}}{1+\Delta t \left( i\xi -i\xi^3 +\gamma(\xi) \right)} \widehat{u_{n+1,r}^{p+1}}. \]
	Hence
	\[ \widehat{u_{n+1,r+1}} - \widehat{u_{n+1}} = \frac{\frac{i\xi \Delta t}{p+1}}{1+\Delta t \left( i\xi -i\xi^3 +\gamma(\xi) \right)} \left( \widehat{u_{n+1}^{p+1}} - \widehat{u_{n+1,r}^{p+1}} \right). \]
	But ,by linearisation around $u_n$
	\begin{align*}
		u_{n+1}^{p+1} - u_{n+1,r}^{p+1} &= \sum\limits_{j=0}^{p} (u_{n+1} - u_{n+1,r}) u_{n+1}^j u_{n+1,r}^{p-j},\\
			& \approx (p+1) (u_{n+1} - u_{n+1,r}) u_n^p.
	\end{align*}
	The end is similar to the Crank-Nicolson scheme.
